Local Differential Privacy for Number of Paths and Katz Centrality

In this paper, we give an algorithm to publish the number of paths and Katz centrality under the local differential privacy (LDP), providing a thorough theoretical analysis. Although various works have already introduced subgraph counting algorithms under LDP, they have primarily concentrated on subgraphs of up to five nodes. The challenge in extending this to larger subgraphs is the cumulative and exponential growth of noise as the subgraph size increases in any publication under LDP. We address this issue by proposing an algorithm to publish the number of paths that start at every node in the graph, leading to an algorithm that publishes the Katz centrality of all nodes. This algorithm employs multiple rounds of communication and the clipping technique. Both our theoretical and experimental assessments indicate that our algorithm exhibits acceptable bias and variance, considerably less than an algorithm that bypasses clipping. Furthermore, our Katz centrality estimation is able to recall up to 90% of the nodes with the highest Katz centrality.

==> proofforglobal.tex <==
\begin{comment}



\section{global algorithm (not used)}

\begin{theorem}
Let $\epsilon \in \mathbb{R}_{\geq 0}$. Let M be a deterministic algorithm of range of input $\mathbb{G}_{n}$ and of input in $\mathbb{R}^{k}$. Let $\sigma \in \mathbb{R}_{> 0}$ such that $\forall i \in [k], M(G)_{i}$ have a sensitivity $\sigma_{i} \leq \sigma$. The two following algorithms provide $\epsilon$-edge DP : \newline
- Noisy argmax : Let $Y = (Y_{1},\dots,Y_{k})$ where the $Y_{i}$ are drawn independently from $Lap(\sigma/\epsilon)$, then output $\argmax_{i \in [k]} (M(G)_{i} + Y_{i})$. \newline 
- Exponential mechanism : Output $i \in [k]$ with probability proportionate to $\exp[\epsilon M_{i}/(2 \sigma)]$.
\end{theorem}

\begin{theorem}
For a graph G  = ([n],E) of maximum degree D and attenuation factor $\alpha \leq 1/D$  the sensitivity $\sigma$ of the whole vector $(Katz(G)[i])_{i \in [n]}$ is : 
\[\sigma \leq \frac{2 \alpha}{(1-\alpha D)^{2}}\]
\end{theorem}

\begin{proof}
By symmetry, we can consider only the case of adding an edge (u,v). We call G' = ([n],E$\cup$(u,v)). We can easily proof by induction that $K(G)^{(i)} \leq (\alpha D)^{i}$. Furthermore for $i \geq 2$,
\[\forall x \in [n]\setminus\{u;v\}, K(G')^{(i)}[x]-K(G)^{(i)}[x] = \alpha \sum_{w \in \eta(x)} K(G')^{(i-1)}[w]-K(G)^{(i-1)}[w] \]
\[K(G')^{(i)}[u]-K(G)^{(i)}[u] = \alpha K(G)^{(i-1)}[v] + \alpha \sum_{w \in \eta(u)} K(G')^{(i-1)}[u]-K(G)^{(i-1)}[u] \]
And the result is symmetric for v. Therefore,
\[\begin{split}
\sum_{x \in [n]} K(G')^{(i)}[x]-K(G)^{(i)}[x] & = \alpha (K(G)^{(i-1)}[u] + K(G)^{(i-1)}[v]) \\ 
& + \alpha \sum_{x \in [n]} \sum_{w \in \eta(x)} K(G')^{(i-1)}[w]-K(G)^{(i-1)}[w] \\
& = \alpha (K(G)^{(i-1)}[u] + K(G)^{(i-1)}[v]) \\
& + \alpha \sum_{w \in \eta(x)} deg(w) (K(G')^{(i-1)}[w]-K(G)^{(i-1)}[w]) \\
& \leq 2 \alpha^{i} D^{i-1} + \alpha D \sum_{x \in [n]} K(G')^{(i-1)}[x]-K(G)^{(i-1)}[x]
\end{split}\]
We know that $\forall x \notin \{u;v\}, K(G')^{(1)}[x] = K(G)^{(1)}[x] $ and $K(G')^{(1)}[u] - K(G)^{(1)}[u] = K(G')^{(1)}[v] - K(G)^{(1)}[v] = \alpha$. Therefore $\sum_{x \in [n]} K(G')^{(1)}[x]-K(G)^{(1)}[x] = 2 \alpha$ and by induction $\forall i \geq 1, \sum_{x \in [n]} K(G')^{(i)}[x]-K(G)^{(i)}[x] \leq 2 i \alpha^{i} D^{i-1}$. Finally : 
\[\begin{split}
|Katz(G')-Katz(G)| & = \sum_{v \in [n]} |Katz(G')[v]-Katz(G)[v]| \\
& = \sum_{v \in [n]} \sum_{i=1}^{\infty} K(G')^{i}[v]-K(G)^{i}[v] \\
& = \sum_{i=1}^{\infty} \sum_{v \in [n]} K(G')^{i}[v]-K(G)^{i}[v] \\
& \leq \sum_{i=1}^{\infty} 2 i \alpha^{i} D^{i-1}
= \frac{2 \alpha}{(1-\alpha D)^{2}}
\end{split}\]
\end{proof}

\textbf{Remark : This upper bound for $\sigma$ is almost tight.}
Indeed we can check by a very similar computation that in a clique of D nodes, the real sensitivity is $\sigma \geq \frac{2 \alpha}{(1-\alpha (D-1))^{2}}$.

\begin{theorem} For a graph G  = ([n],E), of maximum degree D-1 , $x \in [n]$ and attenuation factor $\alpha \leq 1/D$  the sensitivity $\sigma_{x}$ of Katz(G)[i] is : 
\[\sigma_{x} \leq \frac{\alpha}{(1-\alpha D)^{2}} + \frac{2 \alpha^{3} D}{(1-\alpha D)^{2}}\]
\end{theorem}

\begin{proof}
By symmetry, we can consider only the case of removing an edge (u,v). We call $G' = ([n], E \setminus \{(u,v)\})$. In this proof we are going to call \newline $D = \max_{y \in [n]} deg(y)$. If instead of removing an edge we add one, we might increase D by one and therefore need to replace it with D+1.
\[\forall i > 0, \forall y \notin \{u;v\}, K(G)^{i}[y]-K(G')^{i}[y] = \alpha \sum_{z \in \eta(y)} K(G)^{i-1}[z]-K(G')^{i-1}[z]\]
\[\forall i > 0, K(G)^{i}[u]-K(G')^{i}[u] = \alpha K(G)^{i}[v] + \alpha \sum_{z \in \eta(u) \setminus \{v\}} K(G)^{i-1}[z]-K(G')^{i-1}[z]\] 
And the result is the same for v. We notice that the removal of edge (u,v) creates two additional biases $b_{i}(u)$ and $b_{i}(v)$  to $K(G)^{i}[u]-K(G')^{i}[u]$ and $K(G)^{i}[v]-K(G')^{i}[v]$ respectively (at step $i > 0$) with the convention  $\forall y \in [n], K(G)^{(0)}[x] = 1$. This biases then spread to neighbors nodes and cause a bias of $\alpha^{j} (p_{j}(u,x) b_{i}(u) + p_{j}(v,x) b_{j}(v))$ to $K(G)^{i+j}[x]-K(G')^{i+j}[x]$ (at step i+j for $j>0$) with the notation $p_{j}(y,z)$ is the number of paths of length j between y and z in the graph G'. \newline
- We can easily prove by induction that $\forall i> 0, \forall y \in [n], K(G)^{i}[y] \leq (\alpha D)^{i}$ therefore $b_{i}(u) = \alpha K(G)^{i-1}[v] \leq \alpha^{i} D^{i-1}$ and same result for $b_{i}(v)$ \newline 
- We also have $\forall j>0, \forall y \notin \{u;v\}, \forall z \in \{u;v\}, p_{j}(y,z) \leq D^{j-1}$ and \newline 
$\forall j \geq 2, \forall y \in \{u;v\}, \forall z \in \{u;v\}, p_{j}(y,z) \leq D^{j-1}$ and \newline
$\forall y \in \{u;v\}, \forall z \in \{u;v\}, p_{1}(y,z) = 0$. \newline 
Finally  and because $\alpha <1/2,\forall x \notin \{u;v\} : $ 
\[\begin{split}
Katz(G)[x]-Katz(G')[x] & 
\leq \sum_{i = 1}^{\infty} 2 \alpha^{i} D^{i-1} \sum_{j=1}^{\infty} \alpha^{j} D^{j-1} \\
& \leq \sum_{i = 1}^{\infty} 2 \alpha^{i} D^{i-1} (\alpha + \sum_{j=2}^{\infty} \alpha^{j} D^{j-1} )\\
& \leq \frac{2 \alpha^{2}}{1-\alpha D} + \frac{2 \alpha^{3} D}{(1-\alpha D)^{2}}
\leq \frac{\alpha}{1-\alpha D} + \frac{2 \alpha^{3} D}{(1-\alpha D)^{2}}
\end{split}\]
\[\begin{split}
Katz(G)[u]-Katz(G')[u] & \leq \sum_{i = 1}^{\infty} \alpha^{i} D^{i-1} (1 + \sum_{j=2}^{\infty} 2 \alpha^{j} D^{j-1})  \\
& \leq \frac{\alpha}{1-\alpha D} + \frac{2 \alpha^{3} D}{(1-\alpha D)^{2}}
\end{split}\]
The result is the same for v.
\end{proof}

    \begin{algorithm}
    \caption{Clipping Algorithm}\label{euclid}
    \hspace*{\algorithmicindent} \textbf{Input :}
    \text{Graph G = (V,E), attenuation factor $\alpha$, clipping factor X,}
    \text{number of step N} \\
    \hspace*{\algorithmicindent} \textbf{Output : }
    \text{Vector Katz of size $|V|$ storing approximation of Katz}
    \text{centrality of each node}
    \begin{algorithmic}[1]
    \State $\textit{Katz} \gets \textbf{0}^{|V|}$
    \State $ \textit{K}^{(0)} \gets \textbf{1}^{|V|}$
    \For{$i \gets 1$ to N} 
    \State $ \textit{K}^{(i)} \gets \textbf{0}^{|V|}$
    \For{$v \in V$}
    \For{$u \in neighbors(v)$}
    \State $ \textit{K}^{(i)}[v] \gets \textit{K}^{(i)}[v] + \alpha\textit{K}^{(i-1)}[u]$
    \EndFor
    \State $ \textit{Katz[v]} \gets \textit{Katz[v]} + \textit{K}^{(i)}[v]$
    \State $ \textit{K}^{(i)}[v] \gets min(\textit{K}^{(i)}[v],(\alpha X)^{i})$
    \EndFor
    \EndFor
    \State \Return Katz
    \end{algorithmic}
    \end{algorithm}

\begin{lemma}
$\forall x,y \in V, \forall j \geq 2, \forall X>1, p_{j}(x,y) > X^{j} \Rightarrow K^{i+j}[x] > (\alpha X)^{i+j}$
\end{lemma}
\begin{proof}
For $k \leq j$, let $N_{k}$ and $M_{k}$ be respectively the number of path of length k which are part of a path of length j going from x to y and the number of path of length k which are part of a path of length j going from y to x. Therefore $N_{j} = p_{j}(x,y) > X^{j}$ and $M_{j} = p_{j}(x,y) > X^{j}$. Let $A_{1} = N_{1}, B_{1} = M_{1}$ and $\forall 2 \leq k \leq j, A_{k} = N_{k}/N_{k-1}, B_{k} = M_{k}/M_{k-1}$. We have $A_{1} \dots A_{j} = N_{j} > X^{j}$ and $B_{1} \dots B_{j} = M_{j} > X^{j}$.
Therefore $A_{1}B_{j} \dots A_{j}B_{1} > X^{2 j}$, which means there exists $1 \leq k_{0} \leq j$ such that $A_{k_{0}}B_{j+1-k_{0}} > X^{2}$. Here is how we can build a set of path $S_{l}$ for $1 \leq l \leq j+i$ with the invariant that there exist some $k_{l}$ such that every path of $S_{l}$ are at a distance of $k_{l}$ from x on a path of length j to y : \newline
- Let $S_{1}$ = \{all the path of length 1 which are part of a length of path j from x to y\}.
\newline - From $S_{l}$, we either go away from x, which means that we go from the nodes which are at a distance of $k_{l}$ of x on a path from x to y of length j to the nodes which are at a distance of $k_{l} + 1$. This result on $k_{l+1} = k_{l}+1$ and $|S_{l+1}|=A_{k_{l}+1} |S_{l}|$. Or go away from y, which results on $k_{l+1} = k_{l}-1$ and $|S_{l+1}|=B_{j + 1- k_{l}} |S_{l}|$. \newline 
More specifically, - if i = 2 n, then we go away from x for $k_{0}$ step, which results in 
$|S_{k_{0}}| =  A_{1} \dots A_{k_{0}}$ then we go back to x then away from x n times which results in
$|S_{k_{0}+2 n}| = (B_{j+1-k_{0}}A_{k_{0}})^{n} |S_{k_{0}}| > X^{2 n} |S_{k_{0}}|$. Finally we go away from x ($j-k_{0}$) times which results in $|S_{k_{0}+2 n + j - k_{0}}| = |S_{j+i}| = A_{k_{0}+1} \dots A_{j} |S_{k_{0}+2 n}| > X^{2 n} A_{1} \dots A_{j} > X^{i+j}$. \newline 
- if i = 2 n + 1. then we go away from x for $k_{0}$ step, which results in 
$|S_{k_{0}}| =  A_{1} \dots A_{k_{0}}$ then we go back to x then away from x (n+1) times which results in $|S_{k_{0}+2 n + 2}| = (B_{j+1-k_{0}}A_{k_{0}})^{n+1} |S_{k_{0}}| > X^{2 n + 2} |S_{k_{0}}|$. Finally we go away from x ($j-1-k_{0}$) times which results in $|S_{k_{0}+2 n + 2+ j - 1 - k_{0}}| = |S_{j+i}| = A_{k_{0}+1} \dots A_{j-1} |S_{k_{0}+2 n}| > X^{2 n + 2} A_{1} \dots A_{j-1} > X^{i+j+1} > X^{i+j}$. ($A_{j} = 1$ because the last step of any path of length j going from x to y is to get to y, and there is only one way to do so).

\end{proof}


\begin{theorem}
For a graph G of maximum degree D and attenuation factor $\alpha$ and clipping factor X, the sensitivity $\sigma$ of the clipping algorithm is (if $\alpha \leq 1/2)$: 
\[\sigma \leq \frac{\alpha}{1-\alpha X} + \frac{2 \alpha^{3} X^{2}}{(1-\alpha X)^{2}}
\]
\end{theorem}

\begin{proof}
As for the last proof, we consider by symmetry the removal of an edge $(u,v) \in E$ from G = (V,E). Let $G' = (V,E\setminus{(u,v)})$ .We know that this removal creates a bias $b_{i} \leq \alpha (\alpha X)^{i-1}$ at step i for $K^{i}[u]$ and $K^{i}[v]$. This bias then spreads and is responsible for an additional bias of \newline $b_{i,j}(w) \leq \alpha^{j} (p_j(u,w) + p_j(v,w)) b_i$ in $K^{i+j}[w]$. This bias is only added if there is no clipping hence if $K^{i+j}[w] \leq (\alpha X)^{i+j}$. We know that $K^{i+j}[w] \leq (\alpha X)^{i+j}$ implies $\forall y \neq w, p_j(y,w) \leq X^{j}$. Therefore (because $\alpha \leq 1/2)$: 
\[
\begin{split}
Katz(G)[x] - Katz(G')[x] & \leq 
\sum_{i=1}^{\infty} \sum_{j=1}^{\infty} \alpha^{j} (p_j(u,x) + p_j(v,x)) b_i 
\leq \sum_{i=1}^{\infty} \alpha (\alpha X)^{i-1} (2 \alpha + \sum_{j=2}^{\infty} 2 \alpha^{j} X^{j}) \\
& \leq \frac{\alpha}{1-\alpha X}(2 \alpha + \frac{2 \alpha^{3} X^{2}}{(1-\alpha X)^{2}})
\leq \frac{\alpha}{1-\alpha X} + \frac{2 \alpha^{3} X^{2}}{(1-\alpha X)^{2}}
\end{split}
\]
\[
\begin{split}
Katz(G)[u] - Katz(G')[u] & \leq 
\sum_{i=1}^{\infty} b_i (1 + \sum_{j=2}^{\infty} \alpha^{j}(p_j(u,u) + p_j(v,u))) \\
& \leq 
\sum_{i=1}^{\infty} \alpha (\alpha X)^{i-1} (1 + \frac{2 \alpha^{2} X^{2}}{1- \alpha X})
= \frac{\alpha}{1-\alpha X} + \frac{2 \alpha^{3} X^{2}}{(1-\alpha X)^{2}}
\end{split}
\]
The result is the same for v.
\end{proof}

\textbf{Remark : This upper bound for $\sigma$ is almost tight.}
Indeed we can easily check that in a clique of X+1 nodes, then the real sensitivity is $\sigma \geq \frac{\alpha}{1-\alpha X}$. If we set $\alpha = x/X^{2}$ with $x < 1$, we have $\frac{2 \alpha^{3} X^{2}}{(1-\alpha X)^{2}} = \mathcal{O}(\alpha^{2})$,
therefore the theoretical bound gives us $\sigma \leq \frac{\alpha}{1-\alpha X} + \mathcal{O}(\alpha^{2})$.

\subsection{Bias for the global clipping algorithm}
\begin{theorem}

Let $\phi$ be the golden ratio, $Y = max(N,\sqrt{D d})$ and $\alpha < 1/\phi X$ be the attenuation factor. Let $Katz(G)$ be the real Katz value of graph G and $\widetilde{Katz}(G)$ be its estimation by the global clipping algorithm. Then :
\[\forall v \in V, Katz(G)[v] \geq \widetilde{Katz}(G)[v] \]
\[\max_{v \in V} Katz(G)[v] - \widetilde{Katz}(G)[v] \leq 
\frac{\alpha^{2} \phi Y (D-X)}{1- \alpha \phi Y}
\leq \frac{\alpha^{2} \phi X (D-X)}{1-\alpha \phi X}
\]
    
\end{theorem}


\begin{proof}
The first inequality is obvious. We call $K^{i}$ and $\widetilde{K}^{i}$ the intermediate values used in respectively the classic and the clipping algorithm. First of all, let's show by induction that :
\[\forall i \geq 2, \forall v \in V, \max_{v \in V}\widetilde{K}^{i}[v] < (\alpha X)^{i}\]
To do that, we call $M_{i} = \max_{v \in V}\widetilde{K}^{i}[v]$ and 
$m_{i} = \max_{v \in V \mid deg(v) \leq d}\widetilde{K}^{i}[v]$.
We have $M_{1} \leq \alpha X$ (because of the clipping) and $m_{1} \leq \alpha d$. Therefore $\forall v \in V$,
\[\widetilde{K}^{2}[v] = \sum_{u \in \eta(v)} \alpha \widetilde{K}^{1}[u] = \sum_{u \in \eta(v) \mid deg(u) > d} \alpha \widetilde{K}^{1}[u] + 
\sum_{u \in \eta(v) \mid deg(u) \leq d} \alpha \widetilde{K}^{1}[u] \]
\[
\widetilde{K}^{i}[v] \leq \alpha (N K_{1} + D k_{1}) \leq \alpha^{2}(N X + (D - N) d) <
\alpha^{2}(N X + D d) \leq(\alpha X)^{2} 
\]
Hence $M_{2} < (\alpha X)^{2}$. Similarly we can prove that $\forall v \in V, \forall i > 2,
\widetilde{K}^{i}[v] \leq \alpha (N M_{i-1} + D m_{i-1})$ 
hence $M_{i} \leq \alpha (N M_{i-1} + D m_{i-1})$. Furthermore : 
\[
\forall i > 2, \forall v \in V \mid deg(v) \leq d,
\widetilde{K}^{i}[v] = \sum_{u \in \eta(v)} \alpha \widetilde{K}^{i-1}[u] \leq \alpha d M_{i-1}
\]
Which means that $m_{i} \leq \alpha d M_{i-1}$. Therefore $\forall i > 2, M_{i} \leq \alpha N M_{i-1} + \alpha^{2} d D M_{i-2}$. We can now proceed by induction since $M_{1} \leq \alpha X$ and $M_{2} < (\alpha X)^{2}$. Indeed $M_{i-2} 
\leq (\alpha X)^{i-2} X$ and $M_{i-1} < (\alpha X)^{i-1}$ implies \newline $M_{i} < 
\alpha^{i} X^{i-2} (N X + D d) \leq (\alpha X)^{i}$. Thanks to this inequality, we know that the only clipping happens at step one and therefore we have the relation : 
\[
\forall i > 1, \forall v \in V, K^{i}[v] - \widetilde{K}^{i}[v] = 
\sum_{u \in \eta(v)} \alpha (K^{i-1}[u] - \widetilde{K}^{i-1}[u]).
\]
We define $B_{i} = \max_{v \in V} K^{i}[v] - \widetilde{K}^{i}[v] $
and $b_{i} = \max_{v \in V \mid deg(v) \leq d} K^{i}[v] - \widetilde{K}^{i}[v]$.
Using the same technique as above, we show that $\forall i \geq 2, b_{i} \leq \alpha d B_{i-1}$ and 
$B_{i} \leq \alpha (N B_{i-1} + D b_{i-1})$. This means that $\forall i \geq 3,
B_{i} \leq \alpha N B_{i-1} + \alpha^{2} d D B_{i-2}$. We can prove by induction that 
$B_{i} \leq \alpha (D-X) (\alpha \phi Y)^{i-1}$. \newline Indeed $B_{1} = \alpha (D-X)$ and 
$B_{2} \leq \alpha^{2} N (D-X) \leq \alpha^{2} \phi Y (D-X)$. \newline
If we assume $\forall k < i, B_{k} \leq \alpha (D-X) (\alpha \phi Y)^{k-1}$, then \newline
$B_{i} \leq \alpha^{i} (D-X) Y^{i-1} \phi^{i-2} (\phi + 1) = \alpha (D-X) (\alpha \phi Y)^{i-1}$,
which concludes the induction. Finally, to have the bias of the Katz value we add up the biases of all step, except for the first step since this bias comes from clipping and we add $\widetilde{K}^{i}$ to
$\widetilde{Katz}$ before the clipping. The total bias is :
\[\max_{v \in V} Katz(G)[v] - \widetilde{Katz}(G)[v] \leq 
\sum_{i=2}^{\infty} B_{i} \leq \sum_{i=2}^{\infty} \alpha (D-X) (\alpha \phi Y)^{i-1} = 
\frac{\alpha^{2} \phi Y (D-X)}{1- \alpha \phi Y}\]
The last inequality comes from $Y \leq X$ (because $Y = max(N,\sqrt{d D})$ and 
\newline $N X + d D \leq X^{2}$.
\end{proof}
\end{comment}

==> takenfromprel.tex <==
Differential privacy (DP) \cite{dwork2006differential,dwork2014algorithmic} is widely recognized as an optimal method for sharing statistical data from sensitive graphs while maintaining user confidentiality. In our work, we focus on edge differential privacy (edge DP) \cite{hay2009accurate}, which aims to protect the information regarding the presence of an edge connecting two users within the graph. This first kind of differential privacy we present is centralized Differential Privacy (CDP).

\begin{definition}[$\epsilon$-Edge CDP \cite{hay2009accurate}]
For a given $\epsilon \in \mathbb{R}_{\geq 0}$, we say that a randomized algorithm $A$ offers $\epsilon$-edge CDP if, for any pair of input graphs $G,G'$ differing by just a single edge, and any subset S of potential outputs of $A$, the following condition is met:
\[\mathbb{P}[A(G') \in S] \leq \exp(\epsilon) \cdot \mathbb{P}[A(G) \in S].\] \label{def:edgeDP}
\end{definition}

An algorithm offering $\epsilon$-edge CDP guarantees that an adversary can only extract limited information concerning the presence or absence of any edge within the graph. Nevertheless, this model operates on a centralized framework, implying that it assumes the existence of a trusted data aggregator with comprehensive knowledge of the entire graph, responsible for executing the algorithm. Such a model prompts concerns regarding the reliability of the data aggregator as well as the security of the data transmission channel between the aggregator and the users. For these reasons, alternative models like local differential privacy (LDP) \textcolor{blue}{citations} and relationship differential privacy (RDP) \textcolor{blue}{citations} have been proposed. These models aim to protect user privacy without requiring such assumptions. 


\begin{proof}
Let $G$ and $G'$ be graphs differ by a single edge. Suppose that the edge is $(u',v')$. According to Definition \ref{def:edgeLDP}, for all $S_v \subset range(R_v)$, we find that $\mathbb{P}[R_v(a_v') \in S_v] = \mathbb{P}[R_v(a_v) \in S_v]$ for $v \notin \{u',v'\}$, and $\mathbb{P}[R_v(a_v') \in S_v] \leq exp(\epsilon) \cdot \mathbb{P}[R_v(a_v) \in S_v]$ for $v \in \{u',v'\}$. Given that each function $R_v$ is independent, for all $S \subset range(R_{1}) \times \cdots \times range(R_{n})$ and $S_v \subset range(R_v)$, we can state:
\begin{dmath*}
    \mathbb{P}[(R_{1}(a'_{1}),\dots,R_{n}(a'_{n})) \in S] = \prod_{v = 1}^n \mathbb{P}[(R_{v}(a'_{v})) \hiderel{\in} S_v] \leq exp(2\epsilon) \cdot \prod_{v = 1}^n \mathbb{P}[(R_{v}(a_{v})) \hiderel{\in} S_v] = exp(2\epsilon) \cdot \mathbb{P}[(R_{1}(a'_{1}),\dots,R_{n}(a'_{n})) \hiderel{\in} S].
\end{dmath*}
Thus, $(R_{v})_{v \in [n]}$ provides $2 \epsilon$-edge RDP.
\end{proof}

This algorithm can also output every $P_i$ for $i \leq k$ if needed. As we will see in next subsection, this algorithm can be easily adapted to compute Katz centrality. Although the number of paths (and Katz centrality) are global properties which depend on the whole topology of the graph, at each step the calculations done for each node are independent and depend only on the neighbors of this node. This means that this algorithm can be decentralized, which will be necessary for designing a RDP preserving algorithm. 


\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

\Input{Graph $G = ([n],E)$, length of path $k$}
\Output{Vector $P^{(k)}$ of size $n$ where $P^{(k)}[v]$ is the number of paths of length $k$ from node $v \in [n]$ in the graph $G$}
\BlankLine
$P^{(0)} \gets \textbf{1}^{n}$ \;
\For{$i = 1$ \KwTo $k$}{
    \For{$v \in [n]$}{
    $P^{(i)}[v] \gets \sum\limits_{u \in \eta(v)} P^{(i-1)}[u]$ \;
    }
}
\Return $P^{(k)}$
\caption{Computation of paths with a specified length}
 \label{alg:numPaths}
\end{algorithm}
